Adaptive Composite Online Optimization: Predictions in Static and Dynamic Environments

In the past few years, Online Convex Optimization (OCO) has received notable attention in the control literature thanks to its flexible real-time nature and powerful performance guarantees. In this paper, we propose new step-size rules and OCO algorithms that simultaneously exploit gradient predictions, function predictions and dynamics, features particularly pertinent to control applications. The proposed algorithms enjoy static and dynamic regret bounds in terms of the dynamics of the reference action sequence, gradient prediction error, and function prediction error, which are generalizations of known regularity measures from the literature. We present results for both convex and strongly convex costs. We validate the performance of the proposed algorithms in a trajectory tracking case study, as well as portfolio optimization using real-world datasets.

==> style/commands_PM_2.tex <==
%\theoremstyle{theorem}
\newtheorem{Thm}{Theorem}[section]
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Fact}[Thm]{Fact}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{As}[Thm]{Assumption}
\newtheorem{Prb}[Thm]{Problem}
\newtheorem*{pprb}{Problem}

%\theoremstyle{definition}
\newtheorem{Def}[Thm]{Definition}
%\newtheorem*{ddef}{Definition}

%\theoremstyle{remark}
\newtheorem{Rem}[Thm]{Remark}

%\theoremstyle{remark}
\newtheorem{Ex}[Thm]{Example}
%\theoremstyle{definition}
\newtheorem*{nnot}{Notation}
\newcommand{\key}[1]{\textbf{Keywords.} #1}

%======== Abbreviations ==========================
\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}

\newcommand{\PP}{\mathds{P}}
\newcommand{\EE}{\mathds{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Ru}{\overline {\R}}
\newcommand{\Rl}{\underline {\R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\borel}{\mathfrak{B}}

\newcommand{\lra}{\longrightarrow}
\newcommand{\Lra}{\Longrightarrow}
\newcommand{\Lla}{\Longleftarrow}
\newcommand{\Llra}{\Longleftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\da}{\downarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\rra}{\rightrightarrows}

\newcommand{\ind}{\mathds{1}}
\newcommand{\Let}{\coloneqq}
\newcommand{\teL}{\eqqcolon}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\mn}{\wedge}
\newcommand{\mx}{\vee}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\wt}{\widetilde}
\newcommand{\wb}{\widebar}
\newcommand{\shift}{\vartheta}
\newcommand{\com}{\circ}
\newcommand{\tr}{^\intercal}
\newcommand{\opt}{^\star}
\newcommand{\ball}[2]{\mathsf{B}_{#2}(#1)}		%{\mathbb{B}\left(#1;#2\right)}
\newcommand{\ballC}{\overline{\mathsf{B}}}
\newcommand{\ballO}{\mathsf{B}}

\newcommand{\eqsmall}[1]{{\small $#1$}}
\newcommand{\goodgap}{\hspace{\subfigtopskip}}
\newcommand{\note}[1]{\textcolor{red}{(#1)}}

\newcommand{\eps}{\varepsilon}
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\esup}{esssup}
\newcommand{\X}{\mathbb{X}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\conv}{\mathsf{conv}}
%======== More definitions (Optimization) ==========================
\newcommand{\amb}{\mathcal{P}}
\newcommand{\data}{\hat{\xi}}
\newcommand{\Pem}{\widehat{\PP}_N}
\newcommand{\Xiem}{\widehat{\Xi}_N}
\newcommand{\Q}{\mathds{Q}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Lip}{\mathscr{L}}
\newcommand{\dir}[1]{\pmb{\delta}_{#1}}

\newcommand{\Wass}[2]{d_{\mathrm W}\big(#1,#2\big)}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle}
\newcommand{\KL}[2]{d_{\mathrm{KL}}\big(#1,#2\big)}
\newcommand{\TV}[2]{d_{\mathrm{TV}}\big(#1,#2\big)}
\newcommand{\tv}{\mathrm{tv}}

\newcommand{\InfCon}[2]{\overset{#2}{\underset{#1}{\Box}}}
\DeclareMathOperator{\cl}{cl}
\newcommand{\set}[1]{\mathbb{#1}}
\DeclareMathOperator{\st}{s.t.}

%======== ADP ==========================
%\newcommand{\norm}[2]{\left \| #2 \right \|_{#1}}
\newcommand{\Prim}{\mathcal{P}}
\newcommand{\Dual}{\mathcal{D}}
\newcommand{\op}{\mathcal{A}}
\newcommand{\opn}{\mathcal{A}_{n}}
\newcommand{\Jp}{J}
\newcommand{\Jpn}{J_n}
\newcommand{\Jpnd}{J_n(\delta)}
\newcommand{\JpnN}{J_{n,N}}
\newcommand{\Jd}{\wt{J}}
\newcommand{\Jdn}{\wt{J}_n}
\newcommand{\Jdnd}{\wt{J}_n(\delta)}
\newcommand{\cone}{\mathbb{K}}
\newcommand{\leqc}[1]{\preceq_{#1}}
\newcommand{\proj}{\Pi}
\newcommand{\comp}[1]{\overline {#1}}


\newcommand{\Jdnr}{\wt{J}_{n,\eta}}
\newcommand{\Jpnr}{J_{n,\eta}}
\newcommand{\Jpnprime}{J_{\Prim_n^{\prime}}}
\newcommand{\Jpnapprox}{J_{\Prim_{n,\rho,\mu,\kappa}}}
\newcommand{\JDDnprime}{\wt{J}_{n,r}}
\newcommand{\Jac}{J^{\mathrm{AC}}}
\newcommand{\Jdc}{J^{\mathrm{DC}}}

\newcommand{\Jacn}{J^{\mathrm{AC}}_n}
\newcommand{\JacnN}{J^{\mathrm{AC}}_{n,N}}
\newcommand{\Jacnlb}{J^{\mathrm{AC}}_{n,\eta}}
\newcommand{\Jdcn}{J^{\mathrm{DC}}_n}
\newcommand{\JdcnN}{J^{\mathrm{DC}}_{n,N}}

\newcommand{\Jnlb}{J_{n,\eta}^{\rm LB}}
\newcommand{\Jnub}{J_{n,\eta}^{\rm UB}}
\newcommand{\Jneta}{\wt{J}_{n,\eta}}
\newcommand{\Jnetak}{\wt{J}_{n,\eta}^{(k)}}
\newcommand{\Jlb}{J_n^{\rm LB}}

\newcommand{\yeta}{y_{\eta}^{\star}}
\newcommand{\LinOp}{\mathfrak{L}}


\newcommand{\DDual}{\mathcal{DD}}
\newcommand{\xn}{x^\star_n}
\newcommand{\yn}{y^\star_n}
\newcommand{\ynr}{y^\star_{n,\eta}}
\newcommand{\xnN}{x^\star_{n,N}}
\newcommand{\lb}{\underline{\mathfrak{B}}}
\newcommand{\ub}{\overline{\mathfrak{B}}}
\newcommand{\ext}{\mathcal{E}}
\newcommand{\Cont}{\mathcal{C}}
\newcommand{\Prob}{\mathcal{P}}
\newcommand{\Meas}{\mathcal{M}}
\newcommand{\Sigalg}{\mathcal{G}}
\newcommand{\Func}{\mathcal{F}}
\newcommand{\lip}{\mathrm{L}}
\newcommand{\wass}{\mathrm{W}}
\newcommand{\Supp}{\sigma}
\newcommand{\uball}{\mathsf{B}_n}

\newcommand{\ynb}{{\theta_{\mathcal{D}}}}
\newcommand{\xnb}{\theta_{\mathcal{P}}}
\newcommand{\size}[1]{|#1|}
\newcommand{\opQn}{\theta_{n}}
\newcommand{\Rnorm}{\mathfrak{R}}
\newcommand{\Uball}{\U_n}

\newcommand{\cnew}{{\mathbf{c}}}

\newcommand{\wh}{\widehat}

\newcommand{\Nmax}{D_1}
\newcommand{\dmax}{D_2}

\newcommand{\order}{\mathcal{O}}
\newcommand{\bdot}{\LargerCdot}
\newcommand{\ratio}{\varrho_n}
\newcommand{\T}{\mathds{T}}

\newcommand{\Leb}{\lambda}
\newcommand{\Ab}{\mathscr{A}}
\newcommand{\Yb}{\mathscr{Y}}
\newcommand{\Mnorm}{\text{M}}
\newcommand{\cost}{\psi}
\newcommand{\NN}{\mathsf{N}}
\newcommand{\Dac}{\Delta}

\newcommand{\gmax}{g_{\rm max}}
\newcommand{\ie}{{\em i.e.}}
\newcommand{\eg}{{\em e.g.}}

\newcommand{\var}[2][]{V_n^{#1}\!\left[#2\right](k)}
\newcommand{\vark}[2][]{V_n^{#1}\!\left[#2\right]}
\newcommand{\sig}[2][]{\sigma_n^{#1}\left[#2\right](k)}
\newcommand{\sigk}[2][]{\sigma_n^{#1}\left[#2\right]}
\newcommand{\ave}[2][]{\mu_n^{#1}\!\left[#2\right](k)}
\newcommand{\avek}[2][]{\mu_n^{#1}\!\left[#2\right]}
\newcommand{\EZo}[1][]{E(z #1)}
\newcommand{\EZ}[1][]{e}
%\newcommand{\fEZ}[1][]{\widetilde{E}(z #1)}
\newcommand{\fEZ}[1][]{e}
\newcommand{\fa}{f_{{\rm a}}}
\newcommand{\fm}{f_{{\rm m}}}
\newcommand{\hfa}{\widehat{f}_{\rm a}}
\newcommand{\hfm}{\widehat{f}_{\rm m}}
\newcommand{\nsteps}[1]{{#1}_{n}(k)}
\newcommand{\nstepst}[1]{{#1}_{n}^{\intercal}(k)}
\newcommand{\nEZ}{E_{n}(z(k))}
\newcommand{\nfEZ}{\widetilde{E}_{n}(z(k))}
\newcommand{\fmdiag}{f_{m_n}^{\Box}(k)}
\newcommand{\EZdiag}{E_n(z)^{\Box}(k)}
\newcommand{\lpv}{\rho}
\newcommand{\nres}[2][]{\lVert #2 \rVert_{\mathscr{L}_{n #1}}(k)}
\newcommand{\nresk}[2][]{\lVert #2 \rVert_{\mathscr{L}_{n #1}}}
\newcommand{\phact}[1]{\phi_n[#1](k)}
\newcommand{\phactt}[1]{\phi_n^{\intercal}[#1](k)}
\newcommand{\Phact}[1]{\Phi_n[#1](k)}
\newcommand{\Phactps}[1]{\phi_n^\dagger[#1](k)}
\newcommand{\Phactpst}[1]{\phi_n^{\dagger\intercal}[#1](k)}
\newcommand{\Phactt}[1]{\Phi_n^{\intercal}[#1](k)}
\newcommand{\phactf}[1]{\widetilde{\phi}_n[#1](k)}
\newcommand{\phacttf}[1]{\widetilde{\phi}_n^{\intercal}[#1](k)}
\newcommand{\Phactf}[1]{\widetilde{\Phi}_n[#1](k)}
\newcommand{\Phacttf}[1]{\widetilde{\Phi}_n^{\intercal}[#1](k)}

\newcommand{\phactk}[1]{\phi_n[#1]}
\newcommand{\phacttk}[1]{\phi_n^{\intercal}[#1]}
\newcommand{\Phactk}[1]{\Phi_n[#1]}
\newcommand{\Phactpsk}[1]{\phi_n^\dagger[#1]}
\newcommand{\Phactpstk}[1]{\phi_n^{\dagger\intercal}[#1]}
\newcommand{\Phacttk}[1]{\Phi_n^{\intercal}[#1]}
\newcommand{\phactfk}[1]{\widetilde{\phi}_n[#1]}
\newcommand{\phacttfk}[1]{\widetilde{\phi}_n^{\intercal}[#1]}
\newcommand{\Phactfk}[1]{\widetilde{\Phi}_n[#1]}
\newcommand{\Phacttfk}[1]{\widetilde{\Phi}_n^{\intercal}[#1]}

\newcommand{\widebar}[1]{\overline{#1}}
\newcommand{\vecsig}[1]{\mathbf{#1}_n(k)}
\newcommand{\vecsigk}[1]{\mathbf{#1}_n}
\newcommand{\aven}[3][]{\mu_{#3}^{#1}\!\left[#2\right](k)}
\newcommand{\avenk}[3][]{\mu_{#3}^{#1}\!\left[#2\right]}
\newcommand{\varn}[3][]{V_{#3}^{#1}\!\left[#2\right](k)}
\newcommand{\varnk}[3][]{V_{#3}^{#1}\!\left[#2\right]}
\newcommand{\constant}[1]{\mathcal{C}_{#1}}
\newcommand{\shiftop}{\mathfrak{q}}
\newcommand{\step}[1]{\mathfrak{U}_{#1}}
\newcommand{\tf}[1]{\mathcal{#1}}
%\newcommand{\note}[1]{{{\color{red}#1}}



==> style/style_PM_2.tex <==
% ================== Margins & Layout =================================
\addtolength{\voffset}{0cm} 
\addtolength{\textheight}{1cm} 
\addtolength{\hoffset}{-2cm}
\addtolength{\textwidth}{4cm}

\setlength{\parskip}{1mm}
\linespread{1.2}

% \pagestyle{fancy}
% \lhead{}
% \chead[]{}
% \rhead{}

%======== Theorem Environments ===============================
\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{\thesection.\arabic{subsection}}

% ====== Change section title ===============================
\makeatletter
\def\@settitle{\begin{center}%
		\baselineskip14\p@\relax
		\normalfont\LARGE\scshape\bfseries
		%\uppercasenonmath\@title
		\@title
	\end{center}%
}
\makeatother


\makeatletter

%\def\section{\@startsection{section}{1}%
%	\z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
%	{\normalfont\large\bfseries}}

\def\subsection{\@startsection{subsection}{2}%
	\z@{.5\linespacing\@plus.7\linespacing}{.5\linespacing}%
	{\normalfont\large\bfseries}}

\def\subsubsection{\@startsection{subsubsection}{3}%
	\z@{.5\linespacing\@plus.7\linespacing}{.5\linespacing}%
	{\normalfont\itshape}}

% ================== Packages =============
\usepackage[colorlinks	= true,
			raiselinks	= true,
			linkcolor	= MidnightBlue,
			citecolor	= Mahogany,
			urlcolor	= ForestGreen,
			pdfauthor	= {Chris van der Ploeg},
			pdftitle	= {},
			pdfkeywords	= {},   
			pdfsubject	= {},
			plainpages	= false]{hyperref}
\usepackage[usenames, dvipsnames]{color}
\usepackage{dsfont,amssymb,amsmath,subfig, graphicx,fancyhdr,mdframed}
\usepackage{amsfonts,dsfont,mathtools, mathrsfs,amsthm,wrapfig} 
\usepackage[]{siunitx}
\usepackage{ragged2e}
\captionsetup[subfigure]{margin=0pt, parskip=0pt, hangindent=0pt, indention=0pt, 
labelformat=parens, labelfont=rm}
\let\labelindent\relax
\usepackage{enumitem}

\allowdisplaybreaks
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}

% ================== Others =================================
\allowdisplaybreaks
\date{\today}

\patchcmd\@setauthors
  {\MakeUppercase{\authors}}
  {\authors}
  {}{}

